Post-Training Statistical Calibration for Higher Activation Sparsity

We present Statistical Calibrated Activation Pruning (SCAP), a post-training activation pruning framework that (1) generalizes sparsification by input activations of Fully-Connected layers for generic and flexible application across Transformers, and (2) features a simple Mode-Centering technique to pre-calibrate activation distributions for maximizing post-training sparsity. Our results demonstrate robust Pareto efficiency compared to prior methods, translating to a 1.5x additional LLM decoding speedup against CATS at iso model quality. SCAP effectiveness is empirically verified across a wide range of models, including recent Transformer Decoders, MoE, Mamba2, Encoding Transformer, and pre-quantized models, highlighting its practicality and scalability. The code is available at: https://github.com/IntelLabs/SCAP.

==> tables/tab_scap_v_turbosparse.tex <==



==> tables/tab_scap_v_turbosparse_detailed.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{}                                   & \textbf{Mistral-7B-Instruct-v0.2} & \textbf{SCAP}        & \multicolumn{2}{c}{\textbf{TurboSparse}} \\ 
\cmidrule(lr){3-3}\cmidrule(lr){4-5} 
                                            & \textbf{(baseline)}               & \textbf{Up/Gate=30\%} & \textbf{No} & \textbf{With} \\ 
                                            &                                   & \textbf{Down=60\%}    & \textbf{Predictor} & \textbf{Predictor}                      \\ 
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}
\textbf{Input Sparsity}                     &                                   &                        &                          &                          \\ 
Up                                          & -                                 & 32.4                   & -                     & 77.8                        \\ 
Gate                                        & -                                 & 32.4                   & -                     & 77.8                        \\ 
Down                                        & -                                 & 62.3                   & 91.1                     & 91.1                     \\ 
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}
\textbf{FFN}                                & -                                 & \textbf{42.3}          & \textbf{30.4}            & \textbf{82.2}            \\ 
\midrule
\textbf{Optimization}                       &                                   & 1$\times$A100-80GB     & \multicolumn{2}{c}{64$\times$A800-80GB}                       \\ 
\textbf{Infrastructure}                     &                                   &                        &                          &                          \\ 
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}
ARC-challenge                               & 63.0                              & \textbf{63.0}          & 62.2                     & 62.5                     \\ 
Hellaswag                                   & 84.8                              & \textbf{84.5}          & 82.4                     & 82.0                     \\ 
MMLU                                        & 60.8                              & \textbf{60.0}          & 64.4                     & 64.0                     \\ 
TruthfulQA                                  & 68.2                              & \textbf{67.3}          & 52.5                     & 52.6                     \\ 
WinoGrande                                  & 75.5                              & \textbf{75.1}          & 73.2                     & 73.1                     \\ 
GSM8K                                       & 39.0                              & 37.9                   & \textbf{66.7}            & 65.7                     \\
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}
\textbf{OpenLLM}                        &                                   &                        &                          &                          \\ 
\textbf{Leaderboard}                            & 65.2                              & 64.6                   & \textbf{66.9}            & 66.6                     \\ 
\textbf{Avg.}                               &                                   &                        &                          &                          \\ 
\bottomrule
\end{tabular}
\caption{Comparison of input sparsity and performance metrics across different configurations.}
\end{table}

